Mean and median bias reduction in generalized linear models

This paper presents an integrated framework for estimation and inference from generalized linear models using adjusted score equations that result in mean and median bias reduction. The framework unifies theoretical and methodological aspects of past research on mean bias reduction and accommodates, in a natural way, new advances on median bias reduction. General expressions for the adjusted score functions are derived in terms of quantities that are readily available in standard software for fitting generalized linear models. The resulting estimating equations are solved using a unifying quasi-Fisher scoring algorithm that is shown to be equivalent to iteratively re-weighted least squares with appropriately adjusted working variates. Formal links between the iterations for mean and median bias reduction are established. Core model invariance properties are used to develop a novel mixed adjustment strategy when the estimation of a dispersion parameter is necessary. It is also shown how median bias reduction in multinomial logistic regression can be done using the equivalent Poisson log-linear model. The estimates coming out from mean and median bias reduction are found to overcome practical issues related to infinite estimates that can occur with positive probability in generalized linear models with multinomial or discrete responses, and can result in valid inferences even in the presence of a high-dimensional nuisance parameter

==> sections_rev1/glms.tex <==
\IKcomment{This Section will most probably end up having a more
  concise description of GLMs when the final manuscript is ready.}

\subsection{Model}
\label{model} Suppose that $y_1, \ldots, y_n$ are
observations on independent random variables $Y_1, \ldots, Y_n$, each
with probability density or mass function of the exponential family
form
$$
f_{Y_i}(y; \theta_i, \phi) = \exp\left\{\frac{y \theta_i - b(\theta_i) - c_1(y)}{\phi/m_i} - \frac{1}{2}a\left(-\frac{m_i}{\phi}\right) + c_2(y) \right\}
$$
for some sufficiently smooth functions $b(.)$, $c_1(.)$, $a(.)$ and $c_2(.)$, and fixed observation weights $m_1, \ldots, m_n$. The expected value and the variance of $Y_i$ are then
\begin{align*}
      E(Y_i) & = \mu_i =  b'(\theta_i) \\
      Var(Y_i) & = \frac{\phi}{m_i}b''(\theta_i) = \frac{\phi}{m_i}V(\mu_i)
\end{align*}
Compared to the normal distribution, exponential family models are
generally naturally heteroscedastic because the response variance
depends on the mean through the variance function $V(\mu_i)$, and the
dispersion parameter $\phi$ allows shrinking or inflating the
contribution of the mean to the response variance.

A generalized linear model \citep{mccullagh+nelder:1989} links the
mean $\mu_i$ to a linear predictor $\eta_i$ through a a monotone,
sufficiently smooth link function $g(\mu_i) = \eta_i$ with
\begin{equation}
  \label{linear_predictor}
\eta_i = \sum_{t=1}^p \beta_t x_{it}
\end{equation}
where $x_{it}$ is the $(i,t)th$ component of a model matrix $X$, and
$\beta = (\beta_1, \ldots, \beta_p)^\top$. An intercept parameter is
customarily included in the linear predictor, in which case $x_{i1} =
1$ for all $i \in \{1, \ldots, n\}$.

\subsection{Likelihood, score functions and information}
The log-likelihood function for a generalized linear model is
$\sum_{i = 1}^n \log f_{Y_i}(y_i; g^{-1}(\eta_i), \phi)$, where
$g^{-1}(.)$ is the inverse of the link function, and $\eta_i$ is as
in~(\ref{linear_predictor}). Suppressing the dependence of the various
quantities on the model parameters and the data, the derivatives of
the log-likelihood function with respect to the components of $\beta$
and $\phi$ are
\begin{equation}
  \label{scores}
  s_\beta = \frac{1}{\phi}X^TWD^{-1}(y - \mu) \quad \text{and} \quad
  s_\phi = \frac{1}{2\phi^2}\sum_{i = 1}^n (q_i - \rho_i) \, ,
\end{equation}
respectively, with $y = (y_1, \ldots, y_n)^\top$,
$\mu = (\mu_1, \ldots, \mu_n)^\top$,
$W = {\rm diag}\left\{w_1, \ldots, w_n\right\}$ and
$D = {\rm diag}\left\{d_1, \ldots, d_n\right\}$, where
$w_i = m_i d_i^2/v_i$ is the $i$th working weight, with
$d_i = d\mu_i/d\eta_i$ and $v_i = V(\mu_i)$. Furthermore,
$q_i = -2 m_i \{y_i\theta_i - b(\theta_i) - c_1(y_i)\}$ and
$\rho_i = m_i a'_1$ are the $i$th deviance residual and its
expectation, respectively, with $a'_i = a'(-m_i/\phi)$, where
$a'(u) = d a(u)/d u$.

% The only
% `family` object deviating from the above description is `Gamma` where
% `Gamma()$dev.resids` implements $q_i - 2m_i$ instead of
% $q_i$. For convenience in implementation, and just for Gamma we define
% $\rho_i = m_i a'_1 - 2m_i = -2\psi(-m_i/\phi) +
% 2\log(-m_i/\phi)$, where
% $\psi$ is the `digamma` function. This change affects none of the
% estimation methods discussed in this vignette.

The expected information matrix about $\beta$ and $\phi$ is
\begin{equation}
  \label{information}
i =
\left[
\begin{array}{cc}
i_{\beta\beta} & 0_p \\
0_p^\top & i_{\phi\phi}
\end{array}
\right]
=
\left[
\begin{array}{cc}
\frac{1}{\phi} X^\top W X & 0_p \\
0_p^\top & \frac{1}{2\phi^4}\sum_{i = 1}^n m_i^2 a''_i
\end{array}
\right]\,,
\end{equation}
where $0_p$ is a $p$-vector of zeros, and $a''_i = a''(-m_i/\phi)$,
where  $a''(u) = d^2 a(u)/d u^2$.



\subsection{Estimation}

The maximum likelihood estimators $\hat\beta$ and $\hat\phi$ of
$\beta$ and $\phi$, respectively, can be found by the solution of the
score equations $s_\beta = 0_p$ and $s_\phi = 0$. Given that the
dispersion parameter $\phi$ appears in the expression for $s_\beta$
in~(\ref{scores}) only multiplicatively, the maximum likelihood
estimate of $\beta$ can be computed without knowledge of the value of
$\phi$. This fact is exploited in popular software like the
\texttt{glm.fit} function in R \citep{rproject}. The maximum
likelihood estimate for $\hat\phi$ can then be computed in a separate
step by plugging in the estimate for $\beta$, wherever $\beta$ appears
in $s_\psi = 0$ and solving for $\phi$.

The most popular way of computing the maximum likelihood estimate for
$\beta$ is through iteratively reweighted least squares
\citep{green:1984}. Specifically, at the $j$th iteration the current
iterate $\beta^{(j)}$ for $\beta$ is updated by solving the weighted
least squares problem
\begin{equation}
  \label{iwls}
  \left(X^\top W^{(j)} X\right)^{-1} X^\top W^{(j)} z^{(j)}
\end{equation}
where the superscript $(j)$ indicates evaluation at $\beta^{(j)}$, and
$z = (z_1, \ldots, z_n)^\top$ is the vector of ``working'' variates
with $z_i = \eta_i + (y_i - \mu_i)/d_i$. The updated $\beta$ from
weighted least squares problem in \ref{iwls} is equal to the updated
$\beta$ from the Fisher scoring step
$\beta^{(j)} + \left\{i_{\beta\beta}^{(j)}\right\}^{-1}
s_{\beta}^{(j)}$.

\citet{wedderburn:1976} derives necessary and sufficient conditions
for the existence and uniqueness of the maximum likelihood estimator
of $\hat\beta$.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../glmbias"
%%% End:

